Automating a Complete Software Test Process Using LLMs: An Automotive Case Study

Vehicle API testing verifies whether the interactions between a vehicle's internal systems and external applications meet expectations, ensuring that users can access and control various vehicle functions and data. However, this task is inherently complex, requiring the alignment and coordination of API systems, communication protocols, and even vehicle simulation systems to develop valid test cases. In practical industrial scenarios, inconsistencies, ambiguities, and interdependencies across various documents and system specifications pose significant challenges. This paper presents a system designed for the automated testing of in-vehicle APIs. By clearly defining and segmenting the testing process, we enable Large Language Models (LLMs) to focus on specific tasks, ensuring a stable and controlled testing workflow. Experiments conducted on over 100 APIs demonstrate that our system effectively automates vehicle API testing. The results also confirm that LLMs can efficiently handle mundane tasks requiring human judgment, making them suitable for complete automation in similar industrial contexts.

==> includes/dump <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{../figures/api-server-overview.png}
    \caption{An illustration of the in-vehicle API server. When a client issues a GET request to an API like \texttt{/speed}, the server responds with a speed value received as a CAN signal from a speed estimation application. When it receives a PUT request to an API like \texttt{climate}, the server crafts necessary signals and sends it to a climate control application that operates necessary actuators.}
    \label{fig:api-gateway}
\end{figure*}

As illustrated in Figure \ref{fig:api-3demos}, SPAPI follows the typical the 3-tier architecture of decoupling presentation, business logic, and data. Like any other web server, SPAPI presents RESTful endpoints with GET and PUT methods and JSON payloads/responses. In the logic and data layers, however, it differs from the average web server in important ways. First, the typical web server may access data from a database, but `data' for SPAPI is vehicle state information like speed or climate, which are managed by in-vehicle control and monitoring applications. Second, these in-vehicle applications are distributed across several Electronic Control Units (ECUs), interconnected on Controller Area Network (CAN) links. Thus, while the typical web server may access data by executing database queries, SPAPI accesses data by exchanging CAN signals\footnote{A CAN signal is a pre-defined typed quantity sent through a CAN message} with in-vehicle applications. Third, since SPAPI is primarily a gateway, the logic for each endpoint is relatively lean -- it maps API attributes and values into CAN signals and values, before sending them to necessary control applications. Finally, as also shown in Figure \ref{fig:api-3demos}, we focus upon testing SPAPI in a rig, and not in the real vehicle. In the test rig, vehicle state is emulated by a software virtual vehicle (VV) system. Thus, unlike many other API testing settings, VV offers the advantage of being able to freely mock vehicle state. \looseness=-1

For example, the server exposes a \texttt{/speed} API with a GET method that allows a client to read the speed of the vehicle. A client in this case could be an app deployed in an in-vehicle Android tablet. When this client invokes this method, the server picks up the value of a \texttt{VehicleSpeed} CAN signal\footnote{A CAN signal is a pre-defined typed quantity sent through a CAN message} received from, say, a speed estimation application in a vehicle control ECU, and sends it in to the client in the GET response. The \texttt{VehicleSpeed} itself may have originally been estimated using multiple sensors that measure the vehicle speed. Another example is a \texttt{/climate} API with a PUT method that allows a client to adjust the climate settings like the temperature or air conditioning in the cab of the truck. When a client invokes this method to change, say, \texttt{acMode}, the server packs this request into an \texttt{ACModeRequest} CAN signal and sends it to a climate control ECU, which controls necessary actuators to change AC mode. These examples serve to highlight few important characteristics of the in-vehicle API server. 

RESTful API testing constitutes a pivotal element in the realm of software development. It necessitates testers to possess a profound and comprehensive understanding of the relevant domain in order to develop effective test cases. This task becomes particularly intricate when testers are required to comprehend intricate systems such as the CAN signal, alongside mastering various complex systems. The efficacy of these test cases is heavily reliant on such background knowledge, posing a significant challenge for testers to encompass all potential scenarios across diverse APIs.
 
The prevailing automated approaches for RESTful API testing are beset with numerous limitations. These include complexities in usage, challenges in maintenance and updates, a lack of flexibility, and a dependency on precise API documentation for effective test case generation. Furthermore, these methods do not support the incorporation of external knowledge, thereby impacting their overall effectiveness.  

Large Language Models (LLMs) have demonstrated exceptional capabilities in reasoning and code generation. LLM agents can automate these testing tasks with a high degree of proficiency. They are adept at addressing issues using natural language processing, providing robust solutions to the tasks at hand. Additionally, LLM agents offer the flexibility to be seamlessly integrated with external tools, enhancing their functionality and applicability in RESTful API testing.

The SEAPITester must comprehend the definitions of objects within a Swagger file by integrating external knowledge sources, such as CAN signals, and proprietary libraries like 'vv'. Furthermore, it is essential for the SEAPITester to possess the capability to write API test scripts. These scripts are instrumental in generating test case codes tailored for various endpoints. Add examples.

The inherent limitation of Large Language Models (LLMs) is their lack of training on specific knowledge domains, such as the contents of Swagger files and the CAN signals definitions. This raises a critical question: How can we efficiently retrieve and integrate this external domain-specific knowledge into the learning process of an agent?

The test codes generated by our model exhibit significant differences compared to those written by humans. This discrepancy poses a challenge in evaluating the efficacy of our model. Therefore, it is imperative to establish a robust evaluation framework that accurately assesses the quality and functionality of the generated test codes.

Solution approach: Finish all test tasks including test case generation, test execution, and result analysis automatically using a task solving agent. Agent uses LLM for reasoning and is provided with abilities to access info about CAN signals and the private libraries.

\section{Research Questions}

\subsection{RQ 1: What are the effective design and operational strategies for agent-based systems in automated API testing and how do they compare to manual approaches?}

\begin{itemize}
    \item What is a viable architecture for constructing these agents?
    \item What is a viable means for tasking these agents?
    \item What is a viable planning and acting mechanism to achieve the objective of set tasks?
    \item How does an agent-based automatic mechanism compare qualitatively to the manual testing approach?
\end{itemize}

\subsection{RQ2: What are the comprehensive requirements and strategies for agents with the necessary knowledge and tools to effectively conduct testing?}
\begin{itemize}
    \item What kind of external knowledge and tools are necessary for testing?
    \item What are efficient means for providing agents access to required knowledge and tools?
\end{itemize}

\subsection{RQ 3: What are the effective methodologies for assessing the quality and correctness of automatically generated test cases?}
\begin{itemize}
    \item What is a viable mechanism for evaluating the executability (e.g. syntax errors) of automatically generated test cases?
    \item What is a viable mechanism for checking if generated test cases accurately reflect the requirement?
    \item -	What is a viable mechanism for checking if the execution results (pass/fail/error) of generated test cases are interpreted correctly?
\end{itemize}
